Variational Clustering: Leveraging Variational Autoencoders for Image Clustering

Recent advances in deep learning have shown their ability to learn strong feature representations for images. The task of image clustering naturally requires good feature representations to capture the distribution of the data and subsequently differentiate data points from one another. Often these two aspects are dealt with independently and thus traditional feature learning alone does not suffice in partitioning the data meaningfully. Variational Autoencoders (VAEs) naturally lend themselves to learning data distributions in a latent space. Since we wish to efficiently discriminate between different clusters in the data, we propose a method based on VAEs where we use a Gaussian Mixture prior to help cluster the images accurately. We jointly learn the parameters of both the prior and the posterior distributions. Our method represents a true Gaussian Mixture VAE. This way, our method simultaneously learns a prior that captures the latent distribution of the images and a posterior to help discriminate well between data points. We also propose a novel reparametrization of the latent space consisting of a mixture of discrete and continuous variables. One key takeaway is that our method generalizes better across different datasets without using any pre-training or learnt models, unlike existing methods, allowing it to be trained from scratch in an end-to-end manner. We verify our efficacy and generalizability experimentally by achieving state-of-the-art results among unsupervised methods on a variety of datasets. To the best of our knowledge, we are the first to pursue image clustering using VAEs in a purely unsupervised manner on real image datasets.

==> rebuttal.tex <==

We thank the reviewers for their suggestions. Proposed edits shall be made in the camera-ready version if accepted.
%%%%%%%%% BODY TEXT - ENTER YOUR RESPONSE BELOW
%\section{Reviewer \#1}
\subsection{"It's still not clear what's the key difference between the proposed method \& GMVAE"}
\label{ssec:diff_gmvae}



Firstly in GMVAE, the Gaussian prior $\mathbf{z_2}$ depends on a noise variable $\mathbf{z_1}$ \& varies for a given cluster. Ours is more intuitive as it depends only on the cluster. Secondly, GMVAE express the categorical posterior $q(k|\mathbf{z_1},\mathbf{z_2})$ with the prior $p_\beta(\mathbf{z_2}|\mathbf{z_1},k)$ using Bayes' rule. %For doing so, they need to infer the values of $\mathbf{z_1}$ \& $\mathbf{z_2}$ followed by calculating the probability of each cluster. We explicity learn it from the input, making it less computationally intensive \& more effective, as shown in the results. 
Ours is more principled as we learn a one-hot prediction $q(k|\mathbf{z})$ corresponding to a one-to-one mapping between inputs \& cluster assignments rather than a Monte-Carlo estimation from latent variables. This in turn minimizes the reconstruction loss \& KL Divergence between the $\mathbf{z}$ prior \& posterior for just a given cluster instead of over all clusters. This leads to a more effective clustering as seen in the results (Table 1).

\subsection{"It is better to have some toy data results"}

	
\subsection{"Why Haeusser et al do better in MNIST \& STL-10 but much worse in CIFAR10"}

Haeusser et al. perform slightly better only on MNIST. We're better on STL-10 \& much better on CIFAR10. Their large performance discrepancy on similar datasets makes their generalization ability doubtful. Our performance on both these datasets is similar, making it more robust. We refer the reviewer to Pt. \ref{ssec:transfer_learning} to see our transfer learning ability between these datasets.


\subsection{"Will it be able to run in larger dataset"}
\label{ssec:cifar100}

We show results on the FRGCv2 face clustering dataset \& CIFAR100, which has same no. of images as CIFAR10 with 100 classes. FRGCv2 consists of 2462 images having 20 face samples. It's a subset of the larger FRGC dataset. Others report their results on this subset too.


%-------------------------------------------------------------------------
%\section{Reviewer \#2}
%
\setcounter{section}{2}
\setcounter{subsection}{0}
\subsection{"What's the major diff. of proposed method. Major concern is about the novelty"}
	
We refer the reviewer to Pt. \ref{ssec:diff_gmvae} \& \ref{ssec:toy} for differences between us \& GMVAE. The 2$^{nd}$ pt. about $q(k|\mathbf{z})$ applies to VaDE too. VaDE also fix the GMM prior in pre-training. We learn it during training, giving more flexibile learning in an effective way as seen in the results (Table 1). We refer the reviewer to Pt. \ref{ssec:benefit} for our main novelty \& benefit.

	
\subsection{"There is another decoder that learns $\sigma_\theta(\mathbf{z})$"}
	
We don't use another decoder. It's a 2$^{nd}$ output of the decoder $p_\theta(\mathbf{x}|\mathbf{z})$, shown in the appendix (Table A1).

	
\subsection{"Reason for the augmentation loss"}
\label{ssec:aug_imp}
	
As told in Sec. 4.4, augmented images \& aug. loss makes our  robust to varying inputs. This improves the learning, as shown in the ablation study (Appendix Table B1). The augmented \& original images must lie in the same cluster, allowing a "self supervision".

	
\subsection{"Model trained on CIFAR do well on STL"}
\label{ssec:transfer_learning}
	
We show results of this transfer learning below.
	


\subsection{Experiments are somewhat insufficient}
		
	
We refer the reviewer to Pt. \ref{ssec:toy}, \ref{ssec:cifar100} for extra results.
			
%-------------------------------------------------------------------------

%\section{Reviewer \#3}
%
\setcounter{section}{3}
\setcounter{subsection}{0}
\subsection{"How to train the model is not explained. Variational inference is not described."}

The process of Variational Inference is shown in Sec. 3. We expand it with our model in Sec. 4. We show the generation process in Sec. 4.1, inference process in Sec. 4.2, ELBO derivation in Sec. 4.3 \& augmentation in Sec. 4.4. We use Adam optimizer to minimize the loss in Eq. 21, by calculating \& applying gradients w.r.t. network parameters. This shall be made clearer in the final version, if accepted.


\subsection{"How authors did reparameterization"}

We don't explicitly do reparametrization. It's present in newer tensorflow versions(v1.8.0), allowing differentiable low var. sampling to be directly used.


\subsection{"Main benefit of the current method"}
\label{ssec:benefit}

It's in modelling a GMM prior whose params. are learnt during training, which is more flexibile than fixed distributions like in other methods. This is too rigid a constraint mainly in complex datasets (CIFAR/STL). Due to our principled \& effective modelling, acc. on similar datasets are very coherent \& significantly better than others, as seen in our results (Table 1). We perform well even in cross-dataset transfer (Pt. \ref{ssec:transfer_learning}). The benefit of aug. is seen in Pt. \ref{ssec:aug_imp}. 

